Online Learning of Assignments that Maximize Submodular Functions

Which ads should we display in sponsored search in order to maximize our revenue? How should we dynamically rank information sources to maximize value of information? These applications exhibit strong diminishing returns: Selection of redundant ads and information sources decreases their marginal utility. We show that these and other problems can be formalized as repeatedly selecting an assignment of items to positions to maximize a sequence of monotone submodular functions that arrive one by one. We present an efficient algorithm for this general problem and analyze it in the no-regret model. Our algorithm possesses strong theoretical guarantees, such as a performance ratio that converges to the optimal constant of 1-1/e. We empirically evaluate our algorithm on two real-world online optimization problems on the web: ad allocation with submodular utilities, and dynamically ranking blogs to detect information cascades.

==> abstract.tex <==
\begin{abstract}
Which ads should we display in sponsored search in order to maximize our revenue?
How should we dynamically rank information sources to maximize value of information?
These applications exhibit strong diminishing returns: Selection of redundant ads and information sources decreases their marginal utility.
We show that these and other problems can be formalized as
%selecting a partial assignment of items to positions to maximize a monotone submodular utility function. In this paper, we present a novel algorithm for this general problem
%We consider the online problem of
repeatedly selecting an assignment of items to positions to maximize a sequence of \emph{monotone submodular} functions that arrive one by one.
%ANDREAS: Generalizes bandits only in the limited-feedback setting
%This amounts to a generalization of the multiarmed bandit problem in which we must select an element for each position rather than a single element in each round, and the reward function in
%each round is a monotone submodular function of the (element, position)
%pairs we have selected.
%This problem naturally encompasses many
%applications of interest, such as online ad allocation
%under various objective functions and assumptions on user
%behavior, and selecting a list of information sources to query in a
%dynamic environment so as to maximize the value of the information obtained.
We present an efficient algorithm
%with strong theoretical guarantees
for this general problem and analyze it in the \emph{no-regret} model.
%found in the Multiarmed Bandit literature,
%
Our algorithm possesses strong theoretical guarantees, such as a performance ratio that converges to the optimal constant of $1-1/e$. We empirically evaluate our algorithm on two real-world online optimization problems on the web: ad allocation with submodular utilities, and dynamically ranking blogs to detect information cascades.
%We empirically evaluate it on the applications mentioned above.
% (assuming $\P \neq \NP$), and
%are unconditionally optimal in the sense that no algorithm
%with comparable convergence rates can achieve an asymptotic performance ratio
%of $1- 1/e + \epsilon$ for any $\epsilon > 0$, independent of the $\P$ vs. $\NP$ question.
%
%Empirically, we demonstrate that our algorithm

\end{abstract}

%%%%We consider the online problem of repeatedly selecting a partial assignment of elements
%%%to positions to maximize a sequence of monotone submodular functions that arrive
%%%one by one.  This amounts to a generalization of the standard
%%%multiarmed bandit problem in which we must select an element for each position
%%%rather than a single element in each round, and the reward function in
%%%each round is a monotone submodular function of the (element, position)
%%%pairs we have selected.  This problem naturally encompasses many
%%%applications of interest, such as online ad allocation
%%%under various objective functions and assumptions on user
%%%behavior, and selecting a list of information sources to query in a
%%%dynamic environment so as to maximize the value of the information obtained.
%%%We present an efficient algorithm for this problem, analyze it in the
%%%\emph{no-regret} model,
%%%%found in the Multiarmed Bandit literature,
%%%and evaluate it on the applications mentioned above.
%%%%
%%%We prove that our algorithm has a performance ratio that converges to the optimal
%%%constant of $1-1/e$.
%%%% (assuming $\P \neq \NP$), and
%%%%are unconditionally optimal in the sense that no algorithm
%%%%with comparable convergence rates can achieve an asymptotic performance ratio
%%%%of $1- 1/e + \epsilon$ for any $\epsilon > 0$, independent of the $\P$ vs. $\NP$ question.
%%%%



==> algorithm.tex <==


\subsection{The locally greedy algorithm} \label {sec:locally_greedy}

A simple approach to the assignment problem is the following greedy
procedure: the algorithm steps through all $\K$ positions (according
to some fixed, arbitrary ordering). For position $\k$, it simply
chooses the item that increases the total value as much as possible,
i.e., it chooses
\[
s_\k= \argmax_{s \in \Partition_\k} \set { f(\{s_1,\dots,s_{\k-1} \} + s) }\mbox{,}
\]
%(i.e., the item that increases the total value as much as possible).
where, for a set $S$ and element $e$, we write $S + e$ for $S \cup \set{e}$.
Perhaps surprisingly, no matter which ordering over the positions is chosen, this so-called \emph {locally greedy algorithm} produces an assignment that obtains at least half the optimal value~\cite{fisher78}.  In fact, the following more general result holds.  We will use this lemma in the analysis of our improved offline algorithm, which uses the locally greedy algorithm as a subroutine.

%%%%%
\begin {lem} \label {lem:locally_greedy}
Suppose $f : 2^\groundset \to \NonNegativeReals$ is of the form
$f(\assignment) = f_0(\assignment) + \sum_{\k=1}^\K f_\k(\assignment \cap P_\k)$
where $f_0 : 2^\groundset \to \NonNegativeReals$ is monotone submodular, and
$f_\k : P_\k \to \NonNegativeReals$ is arbitrary for $\k \ge 1$.
Let $L$ be the solution returned by the locally greedy algorithm.  Then
$f(L) + f_0(L) \ge \max_{\assignment \in \Feasible} \set { f(\assignment) }$.
\end {lem}
%%%%
\ifthenelse{\boolean{istechrpt}}
{The proof is given in Appendix A.}
{The proof is given in the supplementary material \cite{supplementary}.}
Observe that in the special case where $f_\k = 0$ for all $\k \ge 1$, Lemma \ref
{lem:locally_greedy} says that  $f(L) \ge \frac 1 2 \max_{\assignment \in \Feasible} f(\assignment)$.

The following example shows that the $1/2$ approximation ratio is tight. Consider an instance of the ad allocation problem with two ads, two positions and two users, Alice and Bob. Alice is interested in ad 1, but has a very short attention span: She will only click on the ad if it appears in the first position. Bob is interested in ad 2, and will look through all positions. Now suppose that Alice searches slightly less frequently (with probability $\frac{1}{2}-\varepsilon$) than Bob (who searches with probability $\frac{1}{2}+\varepsilon$). The greedy algorithm first chooses the ad to assign to slot 1. Since the ad is more likely to be shown to Bob, the algorithm chooses ad 2, with an expected utility of $\frac{1}{2}+\varepsilon$. Since Alice will only look at position 1, no ad assigned to slot 2 can increase the expected utility further.  On the other hand, the optimal solution is to assign ad 1 to slot 1, and ad 2 to slot 2, with an expected utility of 1.

\subsection {An algorithm with optimal approximation ratio} \label {sec:offline}

We now present an algorithm that achieves the optimal approximation
ratio of $1 - 1/e$, improving on the $\frac 1 2$ approximation
for the locally greedy algorithm.  Our algorithm associates with each
partition $\Partition_\k$ a \emph {color} $\Color_\k$ from a palette
$\Colors$ of $\NumColors$ colors, where 
we use the notation $\bracket{n}=\set{1,2,\dots,n}$.   
For any set $S \subseteq \groundset \times \Colors$ and vector
$\Colorvec = (\Color_1, \ldots, \Color_\K)$, define\vspace{-2mm}
\[
    \sample_{\Colorvec}(S) = \bigcup_{\k=1}^\K \set { x \in \Partition_\k: (x, \Color_\k) \in S }  \mbox { .}\vspace{-1mm}
\]
Given a set $S$ of (item, color) pairs, which we may think of as
labeling each item with one or more colors, $\sample_{\Colorvec}(S)$
returns a set containing each item $x$ that is labeled with whatever color
$\Colorvec$ assigns to the partition that contains $x$.
Let $F(S)$ denote the expected value of $f(\sample_{\Colorvec}(S))$ when each color $\Color_\k$ is selected uniformly at random from $\Colors$.  We consider the following algorithm.

%%%%%
%\SetKwSty{\textsf}
\SetKw {KwForEach} {for each}
\SetKw {KwFrom} {from}
\SetKw {KwSet} {set}
\SetKw {KwReturn} {return}
\begin {algorithm}
\Titleofalgo { \OfflineGreedy }
\KwIn {integer $\NumColors$, sets $\Partition_1$, $\Partition_2$, \ldots, $\Partition_\K$, function $f: 2^\groundset \to \NonNegativeReals$ (where $\groundset = \bigcup_{\k=1}^\K \Partition_\k$)}
\ \\
\KwSet $G := \emptyset$. \\
%\For(\tcc*[f]{For each color \hspace{1.2em}
%}){\text{\textbf{\emph{each} }} $\Color \in \Colors$}{
\For(\tcc*[f]{For each color \hspace{1.2em} }){$\c$ \KwFrom $1$ \KwTo $\NumColors$}{
  \For(\tcc*[f]{For each partition}){$\k$ \KwFrom $1$ \KwTo $\K$} {
    \KwSet $g_{\k,\c} = \argmax_{x \in \P_\k  \times \set{\c}} \set { F(G
    + x) }$ \tcc*[f]{Greedily pick $g_{\k,\c}$\hspace{0.4em} } \\
    \KwSet $G := G + g_{\k,\c}$\;
  }
}
\KwForEach $\k \in \bracket{\K}$, choose $\Color_\k$ uniformly at random
    from $\Colors$. \\
\KwReturn $\sample_{\Colorvec}(G)$, where  $\Colorvec := (\Color_1, \ldots, \Color_\K)$.
\end {algorithm}
%%%%%
Observe that when $\NumColors = 1$, the $\sample_{\Colorvec}$ function
is deterministic and \OfflineGreedy is simply the locally greedy
algorithm from \secref{sec:locally_greedy}.
In the limit as $\NumColors \to \infty$, the \OfflineGreedy can intuitively be viewed
as an algorithm for a continuous extension of the
problem followed by a rounding procedure, in the
same spirit as Vondr\'{a}k's \emph{continuous-greedy
algorithm}~\cite{calinescu07}.
In our case, the continuous extension is to compute a probability
distribution $D_\k$ for each position $\k$ with support in $P_\k$ (plus
a special ``select nothing'' outcome), such that if we independently
sample an element $x_\k$ from $D_\k$, 
$\E {f(\set{x_1, \ldots, x_\K})}$ is maximized.
% ---------------
It turns out that if the positions individually, greedily, and in
round-robin fashion, add infinitesimal units of probability mass to their
distributions so as to maximize this objective function, they achieve the
same objective function value as if, rather than making decisions in a
round-robin fashion, they had cooperated and added the combination of $\K$
infinitesimal probability mass units (one per position) that greedily maximizes the
objective function.  The latter process, in turn, can be shown to be
equivalent to a greedy algorithm for maximizing a (different) submodular
function subject to a cardinality constraint, which implies that it
achieves a $1-1/e$ approximation ratio~\cite{nemhauser78}.
% ---------------
\ignore{  % old version.
It turns out that if the positions individually, simultaneously, and greedily add probability mass 
at a fixed rate to their distributions to maximize this objective function, they do
nearly as well as a process that adds probability mass
simultaneously at the same rate to all positions in a manner which is greedy with
respect the collective increase in the objective function.
Moreover, the latter process can be viewed as the 
greedy algorithm to maximize a (different) submodular function subject to a 
cardinality constraint~\footnote{More precisely, as the limit process
of the greedy algorithm as $\delta \to 0$, where in each step the
algorithm selects an action that adds $\delta$ probability mass to each $D_\k$, and can perform at most
$1/\delta$ such actions.}, and is thus a $1-1/e$
approximation~\cite{nemhauser78}.
} % end ignore
% --------------
\OfflineGreedy represents a tradeoff between these two extremes;
its performance is summarized by the following theorem. 
%summarizes the performance of \OfflineGreedy.  
For now, we assume that the $\argmax$ in the inner loop is computed exactly.
\ifthenelse{\boolean{istechrpt}}
{In Appendix A}
{In the supplementary material \cite {supplementary},}
we bound the performance loss that results from approximating the $\argmax$
(e.g., by estimating $F$ by repeated sampling).

\begin {thm} \label {thm:offline_greedy}
Suppose $f$ is monotone submodular.  Then
$F(G) \ge \beta(\K, \NumColors) \cdot \max_{\assignment \in \Feasible} \set {f(\assignment)}$,
where $\beta(\K, \NumColors)$ is defined as $1 - (1 - \frac {1} {\NumColors})^{\NumColors} - {\K \choose 2} \NumColors^{-1} $.
\end {thm}

%Observe that as $\J \rightarrow \infty$, the approximation ratio $\beta(\J,
%\K)$ approaches $1 - \frac 1 e$.
It follows that, for any $\varepsilon>0$, \OfflineGreedy achieves a $(1-1/e-\varepsilon)$ approximation factor using a number of colors that is polynomial in $\NumPartitions$ and $1/\varepsilon$.
The theorem will follow immediately from the combination of two key
lemmas, which we now prove.  Informally, Lemma
\ref {lem:outer_loop} analyzes the approximation error due to the
outer greedy loop of the algorithm, while Lemma \ref {lem:inner_loop}
analyzes the approximation error due to the inner loop.

%%%%%
\begin {lem} \label {lem:outer_loop}
Let $G_{\c} = \set { g_{1,{\c}}, g_{2, {\c}}, \ldots, g_{\K, {\c}}  }$, and let $G^-_{\c} = G_1 \cup G_2 \cup \ldots \cup G_{{\c}-1}$.
For each color ${\c}$, choose $E_{\c} \in \Real$ such that
$
  F( G^-_{\c} \cup G_{\c}  )
  \ge \max_{x \in \Rows_{\c}} \set { F(G^-_{\c} \cup x) } - E_{\c}
$
where $\Rows_{\c} := \set{\Row : \forall \k \in \bracket{\K}, |\Row \cap (\P_\k \times \set {{\c}})| = 1}$ is the set of all possible
choices for $G_{\c}$.
%\bigcup_{i=\k}^\K \paren { \P_\k \times \set {{\c}} }$.
Then
\begin {equation} \label {eq:guarantee}
    F(G) \ge \beta(\J) \cdot \max_{\assignment \in \Feasible} \set {f(\assignment)} - \sum_{\j=1}^\J E_\j \mbox { .}
\end {equation}
where $\beta(\J) = 1 - \paren {1 - \frac {1} {\J}}^\J$.
\end {lem}
\begin {proof} [Proof (Sketch)]
We will refer to an element $\Row$ of $\Rows_{\c}$ as a \emph {row}, and to ${\c}$
as the color of the row.  Let $\AllRows := \bigcup_{{\c}=1}^\J \Rows_{\c}$
be the set of all rows.  Consider the function $H:
2^{\AllRows} \to \NonNegativeReals$,
defined as $H(\Rows) = F \paren{ \bigcup_{\Row \in \Rows} \Row }$.  
We will prove the lemma in three steps:
% ---------------------------------
(\emph{i}) $H$ is monotone submodular, 
%
(\emph{ii}) \OfflineGreedy is simply the locally greedy algorithm for finding a
    set of $\K$ rows that maximizes $H$,
where the $\j^{\text{th}}$ greedy step is performed with additive error $E_{\j}$,
    and 
%
(\emph{iii}) \OfflineGreedy obtains the guarantee \eqref
    {eq:guarantee} for maximizing $H$, and this implies the same ratio
    for maximizing $F$.
% ---------------------------------

To show that $H$ is monotone submodular, it suffices to show that $F$ is monotone submodular.  Because $F(\assignment) = \Esub{\Colorvec}{f(\sample_{\Colorvec}(\assignment))}$, and because a convex combination of monotone submodular functions is monotone submodular, it suffices to show that for any particular coloring $\Colorvec$, the function $f(\sample_{\Colorvec}(\assignment))$ is monotone submodular.  This follows from the definition of $\sample$ and the fact that $f$ is monotone submodular.

The second claim is true by inspection.
% Note from Matt: I took this out because you have to understand the argument
% about H vs. f given at the end of the proof before you can see why this is
% true.
%, which implies that \eqref{eq:guarantee} holds with $\beta(\J) = \frac 1 2$.
To prove the third claim, we use the fact that $F(G^-_{\c} \cup \Row)$ can always be
maximized by choosing a row $\Row \in \Rows_{\c}$.  Informally, this is
because $F(G^-_{\c} \cup \Row)$ can always be maximized by choosing a
row whose color has not already been used, and all
colors $\ge {\c}$ are interchangeable.  For problems with this special
property, it is known that the locally greedy algorithm obtains an
approximation ratio of $\beta(\J) = 1 - (1 - \frac 1 \J)^\J$~\cite{nemhauser78}.
Theorem 6 of \cite {streeter07tr} extends this result to handle
additive error, and yields  
\vspace{-2mm}
\[
    F(G) = H( \set {G_1, G_2, \ldots, G_\J} ) \ge \beta(\J) \cdot
\max_{\Rows \subseteq \AllRows: |\Rows| \le \J} \set { H(\Rows) } - \sum_{{\c}=1}^\J E_{\c} \mbox { .}
\vspace{-2mm}\]
To complete the proof, it suffices to show that
$\max_{\Rows \subseteq \AllRows: |\Rows| \le \J} \set { H(\Rows) }
\ge \max_{\assignment \in \Feasible} \set { f(\assignment) } $.  This follows from the
fact that for any assignment $\assignment \in \Feasible$, we can find a set $\Rows(\assignment)$ of $\J$
rows such that $\sample_{\cvec}(\bigcup_{\Row \in \Rows(\assignment)} R) = \assignment$ with
probability 1, and therefore $H(\Rows(\assignment)) = f(\assignment)$.
\end {proof}

We now bound the performance of the the inner loop of \OfflineGreedy.

\begin {lem} \label {lem:inner_loop}
Let $f^* = \max_{\assignment \in \Feasible} \set {f(\assignment)}$,
and let $G_{\c}$, $G^-_{\c}$, and $\Rows_{\c}$ be defined as in the statement of Lemma \ref
{lem:outer_loop}.  Then, for any ${\c} \in \bracket{\J}$,
\[
    F (G^-_{\c} \cup G_{\c}) \ge \max_{\Row \in \Rows_{\c}} \set {
    F(G^-_{\c} \cup \Row) } -  {\K \choose 2} \J^{-2} f^*
%    - \sum_{i=1}^\K \eps_{i,{\c}}
    \mbox { .}
\]
\end {lem}

\begin {proof} [Proof (Sketch)]
Let $N$ denote the number of partitions whose color is ${\c}$.  
For $\Row \in \Rows_{\c}$, let
$\Delta_{\cvec}(\Row) := f(\sample_{\cvec}(G^-_{\c} \cup \Row)) -
f(\sample_{\cvec}(G^-_{\c}))$, and let $F_{\c}(\Row) := F(G^-_{\c} \cup \Row) - F(G^-_{\c})$.  By definition,
%\[
    $F_{\c}(\Row) = \Esub{\cvec}{\Delta_{\cvec}(\Row)} = \Pr{N=1} \Esub{\cvec} {  \Delta_{\cvec}(\Row)  | N = 1 } + \Pr{N \ge 2} \Esub{\cvec}{\Delta_{\cvec}(\Row) | N \ge 2}$,
%\]
where we have used the fact that $\Delta_{\cvec}(\Row) = 0$ when $N =
0$.
% for $\Row \in \Rows_{\c}$.
The idea of the proof is that the first of these terms dominates as
$\J \to \infty$, and that $ \Esub{\cvec} {  \Delta_{\cvec}(\Row)  | N = 1 }$
%$\Delta_{\cvec}(\Row)$ can
%be optimized exactly when $N = 1$ 
can be optimized exactly
simply by optimizing each element of
$P_\k \times \set{{\c}}$ independently.
Specifically, it can be seen that $\Esub{\cvec}{  \Delta_{\cvec}(\Row)  | N = 1 } =
\sum_{\k=1}^\K f_\k(\Row \cap (P_\k \times \set{{\c}}))$ for suitable $f_\k$.
Additionally, $f_0(\Row) = \Pr{N \ge 2} \Esub{\cvec}{\Delta_{\cvec}(\Row) | N \ge
2}$ is a monotone submodular function of a set of (item, color) pairs, for the same reasons $F$ is.
Applying Lemma \ref {lem:locally_greedy} with these 
%choices for
$\set{f_\k : \k \ge 0}$ yields
\[
    F_{\c}(G_{\c}) + \Pr{N \ge 2} \Esub{\cvec}{\Delta_{\cvec}(G_{\c}) | N \ge 2} \ge \max_{R \in \Rows_{\c}} \set { F_{\c}(R) }
    %- \sum_{\k=1}^\K \eps_{\k,{\c}}
    \mbox { .}
\]
To complete the proof, it suffices to show that $\Pr{N \ge 2} \le {K
\choose 2} \J^{-2}$ and that $\Esub{\cvec}{\Delta_{\cvec}(G_{\c}) | N \ge 2}
\le f^*$.
The first inequality holds because, if we let $M$ be the number of \emph{pairs} of partitions that are both assigned color ${\c}$, we have $\Pr{N \ge 2} = \Pr{M \ge 1}\le \E{M} = {\K \choose 2} \J^{-2}$.
%The first inequality follows from three facts:
%$N \ge 2$ implies a pair of partitions are both assigned color ${\c}$, the expected number of such pairs is ${\K \choose 2} \J^{-2}$, and Markov's inequality.
The second inequality follows from the fact that for any
$\cvec$ we have $\Delta_{\cvec}(G_{\c}) \le f(\sample_{\cvec}(G^-_{\c} \cup G_{\c})) \le
f^*$.
\end {proof}

%Combining lemmas \ref {lem:outer_loop} and \ref {lem:inner_loop} proves
%Theorem \ref {thm:offline_greedy}.


==> conclusions.tex <==
\vspace{-2mm}\section{Conclusions}\vspace{-2mm}
\label{sec:conclusions}
In this paper, we showed that important problems, such as ad display in
sponsored search and computing diverse rankings of information sources
on the web, require optimizing assignments under submodular utility
functions. We developed an efficient algorithm, \OfflineGreedy, which
obtains the optimal approximation ratio of $(1-1/e)$ for
this NP-hard optimization problem.  We also developed an online
algorithm, \OnlineGreedy, that asymptotically achieves no
$(1-1/e)$-regret for the problem of repeatedly selecting informative
assignments, under the full-information and bandit-feedback
settings.  Finally, we demonstrated that our algorithm outperforms 
previous work 
%existing techniques 
on two real world problems, namely online ranking of
informative blogs and ad allocation.


==> evaluation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Implementation details} % [Andreas]
We evaluate \OnlineGreedy experimentally on two applications: Learning to rank blogs that are effective in detecting cascades of information, and allocating advertisements to maximize revenue.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Online learning of diverse blog rankings} % [Andreas]
We consider the problem of ranking a set of blogs and news sources on the web.
Our approach is based on the following idea: A blogger writes a posting, and, after some time, other postings link to it, forming cascades of information propagating through the network of blogs.
%Such information cascades model the spread of stories through the blogosphere, and the goal is to select blogs which detect the biggest stories as early as possible.

More formally, an information cascade is a directed acyclic graph of vertices
(each vertex corresponds to a posting at some blog), where edges are
annotated by the time difference between the postings.
Based on this
notion of an information cascade, we would like to select blogs
that detect big cascades (containing many nodes) as early as
possible (i.e., we want to learn about an important event before
most other readers). In
\cite{leskovec07}
%\cite{leskovec07cost}
 it is shown how one
can formalize this notion of utility using a monotone submodular function
that measures the informativeness of a subset of blogs. Optimizing the submodular function yields a small set of blogs that ``covers'' most cascades.  This utility function prefers \emph{diverse} sets of blogs, minimizing the overlap of the detected cascades, and therefore minimizing redundancy.
% Due to space limitations, we refer to \cite{leskovec07} for a formal definition of $g$.

The work by \cite{leskovec07} leaves two major shortcomings: Firstly, they select a \emph{set} of blogs rather than a \emph{ranking}, which is of practical importance for the presentation on a web service. Secondly, they do not address the problem of \emph{sequential} prediction, where the set of blogs must be updated dynamically over time. In this paper, we address these shortcomings.

%\paragraph{Data set}

\paragraph{Results on offline blog ranking.}
\newcommand {\Blogs} {\mathcal{B}}
In order to model the blog ranking problem, we adopt the assumption that different users have different attention spans: Each user will only consider blogs appearing in a particular subset of positions. In our experiments, we assume that the probability that a user is willing to look at position $\k$ is proportional to $\gamma^\k$, for some discount factor $0<\gamma<1$.
More formally, let $g$ be the monotone submodular function measuring the informativeness of any set of blogs, defined as in \cite{leskovec07}.
Let $\Partition_\k = \Blogs \times \set {\k}$, where $\Blogs$ is the set of blogs.  Given an assignment $S \in \Feasible$, let $S^{[\k]} = S \cap \set { \Partition_1 \cup \Partition_2 \cup \ldots \cup \Partition_\k }$ be the assignment of blogs to positions 1 through $\k$.
We define the \emph{discounted} value of the assignment $S$ as
$
f(S) = \sum_{\k=1}^\K \gamma^\k \paren{ g(S^{[\k]})-g(S^{[\k-1]}) }.
$
It can be seen that $f: 2^\groundset \to \NonNegativeReals$ is monotone submodular.

For our experiments, we use the data set of \cite{leskovec07}, consisting of 45,192 blogs, 16,551 cascades, and 2 million postings collected during 12 months of 2006. We use the \emph{population affected} objective of \cite{leskovec07}, and use a discount factor of $\gamma = 0.8$.
Based on this data, we run our \OfflineGreedy algorithm with varying numbers of colors $\NumColors$ on the blog data set. \figref{fig:blogs_offline} presents the results of this experiment. For each value of $\NumColors$, we generate 200 rankings, and report both the average performance and the maximum performance over the 200 trials. Increasing $\NumColors$ leads to an improved performance over the locally greedy algorithm ($\NumColors=1$).

%One of the major issues identified by \cite{leskovec07cost} is that optimizing the selection on historic data can lead to poor generalization to unseen test data. In this paper, we use our algorithm to address this shortcoming.

\paragraph{Results on online learning of blog rankings.}

We now consider the online problem where on each round $t$ we want to output a ranking $S_t$. After we select the ranking, a new set of cascades occurs, modeled using a separate submodular function $f_t$, and we obtain a reward of $f_t(S_t)$. In our experiments, we choose one assignment per day, and define $f_t$ as the utility associated with the cascades occurring on that day. Note that $f_t$ allows us to evaluate the performance of any possible ranking $S_t$, hence we can apply \OnlineGreedy in the \emph{full-information feedback} model.

We compare the performance of our online algorithm using $\NumColors =
1$ and $\NumColors = 4$. \figref{fig:blogs_discount} presents the
average cumulative reward gained over time by both algorithms. We
normalize the average reward by the utility achieved by
the \OfflineGreedy algorithm (with $\NumColors = 1$) applied to the
entire data set.  \figref{fig:blogs_discount} shows that the
performance of both algorithms rapidly (within the first
47 rounds) converges to the performance of the offline
algorithm. The \OnlineGreedy algorithm with $\NumColors = 4$ levels
out at an approximately 4\% higher reward than the
algorithm with $\NumColors=1$.

%Since blogs from
%different topics (such as politics, religion, tech news, etc.)
%participate in different cascades. , the solution set $\cA$ will
%typically contain very \emph{diverse} blogs. Similar blogs that
%overlap significantly suffer from diminishing returns.



% TODO: the horizontal axis on figure (b) should use "Rounds" instead of "Time Steps"
\begin{figure}[t]
\centering
%\subfigure[b]{
\subfigure[Blogs: Offline results]{
\includegraphics[width=.31\textwidth]{fig/experiment_offline_discount45k}
%\includegraphics[width=.4\textwidth]{fig/todo}
 \label{fig:blogs_offline}
 }
% \subfigure[a]{
 \subfigure[Blogs: Online results]{
%\includegraphics[width=.4\textwidth]{fig/todo}
\includegraphics[width=.31\textwidth]{fig/experiment_online_discount1k_performance}
 \label{fig:blogs_discount}
 }
 \subfigure[Ad display: Online results]{
%\includegraphics[width=.4\textwidth]{fig/todo}
\includegraphics[width=.31\textwidth]{fig/experiment_online_ads_markovian_users}
\label{fig:online_ads}
 }
\caption{\small (a,b) Results for discounted blog ranking ($\gamma = 0.8$), in offline (a) and online (b) setting. (c) Performance of \OnlineGreedy with $\J = 1$,
$2$, and $4$ colors for the sponsored search ad selection problem (each round is a query).  Note that $\J = 1$ corresponds to the online
algorithm of~\cite {radlinski08, streeter08}.\vspace{-4mm}}
\end{figure}
%\vspace{-1em}


% ===============================================
\subsection{Online ad display} \label{ssec:online_ads}
% ===============================================
\newcommand {\Ads} {\mathcal{A}}
\newcommand {\Pclick}{\ensuremath{p_{\text{click}}}}
\newcommand {\Pabandon}{\ensuremath{p_{\text{abandon}}}}

We evaluate \OnlineGreedy for the sponsored search ad selection
problem in a simple Markovian model incorporating the value of diverse results and
complex position-dependence among clicks.
In this model, each user $u$ is defined by
two sets of probabilities:
$\Pclick(a)$ for each ad $a \in \Ads$, and $\Pabandon(\k)$ for each
position $\k \in \bracket{\K}$.  When presented an assignment of ads
$\set{a_1, a_2, \ldots, a_\K}$, where $a_\k$ occupies position $\k$,
the user scans the positions in increasing order.
For each position $\k$, the user clicks on $a_\k$ with probability
$\Pclick(a_\k)$, leaving the results page forever.
Otherwise, with probability $(1 - \Pclick(a_\k)) \cdot \Pabandon(\k)$, the user loses interest and
abandons the results without clicking on anything.
Finally, with probability $(1 - \Pclick(a_\k)) \cdot (1 - \Pabandon(\k))$, the user proceeds to look
at position $\k+1$.
The reward function $f_t$ is the number of clicks, which is either zero or
one. We only receive information about $f_t(S_t)$ (i.e., \emph{bandit feedback}).


In our evaluation, there are two types of users: those interested in
all positions ($\Pabandon \equiv 0$), and those that quickly
lose interest ($\Pabandon \equiv 0.5$).  For both types of users we
select $\Pclick(a)$ uniformly at random from $[0, 1]$, independently
for each ad $a$ (once chosen, $\Pclick$ is fixed for all rounds).  We use $\K = 6$ positions, and 6 available ads.
%We will evaluate \OnlineGreedy on this application in terms of the
%click-through rate it achieves.  For each query, we draw the pair
%$(\Pclick, \Pabandon)$ from some distribution (to be determined).
In~\figref{fig:online_ads} we compare the performance of \OnlineGreedy with $\J = 4$ to the online
algorithm of~\cite {radlinski08, streeter08}, based on the average of 100 experiments.  The latter algorithm is
equivalent to running \OnlineGreedy with $\J = 1$.  The former achieves parity with the latter
after roughly $10^6$ rounds, and dominates thereafter.
% achieving roughly a 1\% improvement in click-through rates relative to~\cite {radlinski08,
%streeter08} by $10^7$ rounds.


It can be shown that with several different types of users with
distinct $\Pclick(\cdot)$ functions the
offline problem of finding an assignment within
$1 - \frac 1 e + \eps$ of optimal is $\NP$-hard.
This is in contrast to the
case in which $\Pclick$ and $\Pabandon$ are the \emph {same} for all
users; in this case the offline problem simply requires finding an
optimal policy for a Markov decision process, which can be done
efficiently using well-known algorithms.
A slightly different Markov model of user behavior which is efficiently solvable was considered in~\cite{aggarwal08}.
In that model, $\Pclick$ and $\Pabandon$ are the same for all users, and
$\Pabandon$ is a function of the ad in the slot currently being
scanned rather than its index.


%\begin{figure}[t]
%\centering
%\includegraphics[width=.45\textwidth]{fig/experiment_online_ads_markovian_users}
%\label{fig:online_ads}
%\caption{
%\small Performance of \OnlineGreedy with $\J = 1$,
%$2$, and $4$ colors for the sponsored search ad selection input distribution
%described above.  Note $\J = 1$ corresponds to the online
%algorithm of~\cite {radlinski08, streeter08}.  Each round is a query.
%%of \S~\ref{ssec:online_ads}
%} % end caption
%\end{figure}


==> intro.tex <==
\vspace{-2mm}
\section{Introduction} \label{sec:intro}
\vspace{-1mm}
% ---------------------------------------------------------------------------------

Consider the problem of repeatedly choosing advertisements to display in sponsored search to maximize our revenue.  In this problem, there is a small set of positions on the page, and each time a query arrives we would like to assign,
to each position,
one out of a large number of possible ads.  In this and related problems that we call \emph{online assignment learning} problems,
there is a set of positions, a set of items, and a sequence of rounds, and on each round we must assign an item to each position.  After each round, we obtain some reward
depending on the selected assignment, and we observe the value of the reward.  When there is only one position, this problem
becomes the well-studied multiarmed bandit problem~\cite{auer2002}.
When the positions have a linear ordering
the assignment can be construed as a ranked list of elements, and the
problem becomes one of selecting lists online.
Online assignment learning thus models a central challenge in web
search, sponsored search, news aggregators, and recommendation
systems, among other applications.

%In these applications, the algorithm is faced with a stream of
%user queries, and must learn about user
%behavior over time.
A common assumption made in previous work on these problems is that the quality of an assignment is the sum of a function on the (item, position) pairs in the assignment.  For example, online advertising models with \emph {click-through-rates}~\cite{edelman07a} make an assumption of this form.
More recently, there have been attempts to incorporate
the value of diversity in the reward function~\cite{radlinski08}.
Intuitively, even though the best $\NumPartitions$ results for the
query ``turkey'' might happen to be about the country, the best list
of $\NumPartitions$ results is likely to contain some recipes for the
bird as well.  This will be the case if there are diminishing returns
on the number of relevant links presented to a user;
for example, if it is better to present each user with at least one relevant result
than to present half of the users with no relevant results and half with
two relevant results.
We incorporate these considerations in a flexible way by providing an algorithm that performs well whenever the reward for an assignment is a \emph{monotone submodular
function} of its set of (item, position) pairs.

Our key contributions are:
(\emph{i}) an efficient algorithm, \OfflineGreedy, that provides a constant factor $(1-1/e)$ approximation to the problem of optimizing assignments under submodular utility functions,
(\emph{ii}) an algorithm for online learning of assignments, \OnlineGreedy, that has strong performance guarantees in the \emph {no-regret} model, and
%(discussed below)
(\emph{iii}) an empirical evaluation on two problems of information gathering on the web.

% ---------------------------------------------------------------------------------
\section{The assignment learning problem} %, Models, \& Assumptions}
\label{sec:problem}
% ---------------------------------------------------------------------------------

We consider problems, where we have $\NumPartitions$ positions (e.g., slots for displaying ads), and need to assign to each position an item (e.g., an ad) in order to maximize a utility function (e.g., the revenue from clicks on the ads).  We address both the \emph{offline} problem, where the utility function is specified in advance, and the \emph{online} problem, where a sequence of utility functions arrives over time, and we need to repeatedly select a new assignment.

%=======
%\paragraph{The Offline Problem.} In the offline problem we are given as input sets
%set $\Partition_1$, $\Partition_2$, \ldots, $\Partition_\NumPartitions$,
%where $\Partition_i$ is the set of elements that may be placed
%in position $i$.  We assume without loss of generality that these sets are disjoint.  A set containing at most  one element from each $\Partition_i$ is termed a \emph {feasible assignment}; we use $\Feasible$ to denote the set of feasible assignments.
%Our goal is to select a feasible assignment $S \in \Feasible$ that maximizes a monotone submodular function $f:2^\groundset \to \NonNegativeReals$, where $\groundset = \bigcup_{i=1}^\NumPartitions \Partition_i$.  As discussed in \S \ref {sec:related_work}, this problem is an instance of maximizing a monotone submodular function subject to a (simple) partition matroid constraint.\\

\paragraph{The Offline Problem.}
In the offline problem we are given sets $\Partition_1$, $\Partition_2$, \ldots, $\Partition_\NumPartitions$, where $\Partition_\k$ is the set of items that may be placed
in position $\k$.  We assume without loss of generality that these sets are disjoint.\footnote{If the same item can be placed in multiple positions, simply create multiple distinct copies of it.} An \emph{assignment} is a subset $\assignment\subseteq\groundset$, where $\groundset=\Partition_1\cup\Partition_2 \cup \dots\cup\Partition_\NumPartitions$ is the set of all items.
We call an assignment \emph{feasible}, if at most one item is assigned to each position (i.e., for all  $\k$, $|\assignment \cap \Partition_\k| \le 1$).  We use $\Feasible$ to refer to the set of feasible assignments.

Our goal is to find a feasible assignment maximizing a utility function $f:2^{\groundset}\to\NonNegativeReals$.
As we discuss later, many important assignment problems satisfy \emph{submodularity}, a natural diminishing returns property:  Assigning a new item to a position $\k$ increases the utility more if few elements have been assigned yet, and less if many items have already been assigned.  Formally, a utility function $f$ is called submodular, if for all $\assignment\subseteq\assignment'$ and $s\notin\assignment'$ it holds that
$f(\assignment\cup\set{s})-f(\assignment)\geq f(\assignment'\cup\set{s})-f(\assignment')$. We will also assume $f$ is monotone (i.e., for all $\assignment\subseteq\assignment'$, we have $f(\assignment)\leq f(\assignment')$).  Our goal is thus, for a given non-negative, monotone and submodular utility function $f$, to find a feasible assignment $\assignment^*$ of maximum utility, $\assignment^*=\argmax_{\assignment\in\Feasible}\set{f(\assignment)}$.
% Notes from Matt:
% * we want to allow different sets of elements to be eligible for different positions
% * in the ads application, the elements of \Partition_i would be (ad, position) pairs
% * by defining the function of be non-negative, we avoid the need to assume f(\emptyset) = 0.

This optimization problem is NP-hard. In fact, a stronger negative result holds:
\begin{thm}[\cite{mirrokni08}]\label{thm:hardness}
For any $\epsilon > 0$, any algorithm guaranteed to obtain a solution within a
factor of $(1-1/e + \epsilon)$ of $\max_{\assignment\in\Feasible}
\set { f(\assignment) }$
requires exponentially many evaluations of $f$ in the worst case.
\end{thm}
In light of this negative result, we can only hope to obtain a solution that achieves a fraction of $(1-1/e)$ of the optimal value. In \secref{sec:offline} we develop such an algorithm.

%=======
\paragraph{The Online Problem.}
The offline problem is inappropriate to model dynamic settings, where
the utility function may change over time, and we need to repeatedly
select new assignments, trading off exploration (experimenting with ad
display to gain information about the utility function), and
exploitation (displaying ads which we believe will maximize utility).
More formally, we face a sequential decision problem, where,
%Then, queries $\set{q_\roundindex}_{\roundindex \ge 1}$ arrive one by one, each
%associated with a monotone submodular reward function
%$f_{\roundindex}: 2^\groundset \to [0,1]$
%\andreas{not so sure about this ``queries'' formulation -- it looks like we want to take information about the query into account, as in the contextual bandits}.
on each round (which, e.g., corresponds to a user query for a
particular term), we want to
select an assignment $\assignment_{\roundindex}$ (ads to display).  We
assume that the sets $\Partition_1$, $\Partition_2$, \ldots,
$\Partition_\NumPartitions$ are fixed in advance for all
rounds.
%\andreas{need to comment on that assumption}
After we select
the assignment we obtain reward
$f_{\roundindex}(\assignment_{\roundindex})$ for some monotone
submodular utility function $f_{\roundindex}$.  We call the setting
where we do not get any information about $f_{\roundindex}$ beyond the
reward the \emph{bandit feedback} model.
%
%$f_{\roundindex}$
%Before gaining any information about $f_{\roundindex}$,
%we must select a feasible assignment $\assignment_{\roundindex}$; we then receive a reward $f_{\roundindex}(\assignment_{\roundindex})$.
In contrast, in the \emph{full-information feedback} model we obtain
oracle access to $f_{\roundindex}$ (i.e., we can evaluate
$f_{\roundindex}$ on arbitrary feasible assignments).
Both models arise in real applications, as we show in \secref{sec:evaluation}.

\ignore{
\begin{enumerate}
\item \emph{Constrained Full Information.}
 %After selecting $S_{\roundindex}$,
  We obtain
  oracle access to $f_{\roundindex}$, meaning we may obtain
  $f_{\roundindex}(\assignment)$ for any set $\assignment \in \Feasible$ (but not for $\assignment
  \notin \Feasible$).
\item \emph{Partial Information.} %After selecting $\assignment_{\roundindex}$,
  We see the values
  $\set{f_{\roundindex}(\assignment_{\roundindex}^{\k}) :
    \k \in \bracket{\NumPartitions} }$, where
$\assignment_{\roundindex}^{\k} :=
\bigcup_{\k' \in \bracket{\k}} \paren{
  \assignment_{\roundindex} \cap P_{\k'} }$.
%$\assignment_{\roundindex}^{\k} := \assignment_{\roundindex} \cap
%  (\listgroundset \times \bracket{\k}) $.
\item \emph{Bandit Feedback.} We get no additional information beyond $f_{\roundindex}(\assignment_{\roundindex})$.
\end{enumerate}
} % end ignore

The goal is to maximize the total reward we obtain, namely
$\sum_{\roundindex} f_{\roundindex}(\assignment_{\roundindex})$.
Following the multiarmed bandit
literature, we evaluate our performance after $\NumRounds$ rounds by comparing our
total reward against that obtained by a clairvoyant algorithm with
knowledge of the sequence of functions $\tuple{f_1, \ldots, f_{\NumRounds}}$,
but with the restriction that it must select the same assignment
on each round.
%restrictions on how often it can change its output set
%$\assignment_{\roundindex}$.
The difference between the clairvoyant algorithm's total reward and
ours is called our \emph{regret}.
%The most common restriction is to require the algorithm to select the same
%assignment in each round.
The goal is then to develop an algorithm whose
expected regret grows sublinearly in the number of rounds; such an algorithm is
said to have (or be) \emph{no-regret}.
However, since sums of submodular functions remain submodular, the clairvoyant algorithm has to solve an offline assignment problem with $f(\assignment)=\sum_{\roundindex} f_{\roundindex}(\assignment)$. Considering \thmref{thm:hardness}, no polynomial-time algorithm can possibly hope to
achieve a no-regret guarantee. % because the underlying offline problem requires exponentially many oracle calls to the submodular function to approximate to within a
%factor of $(1-1/e + \epsilon)$ for any $\epsilon > 0$~\cite{mirrokni08}.
To accommodate this fact, we discount the reward of the clairvoyant algorithm by a factor of
$(1-1/e)$: We define the
%\begin{defn}  The
\emph{$(1-1/e)$-regret} of a random sequence
  $\tuple{\assignment_1, \ldots, \assignment_{\NumRounds}}$ %, or of a randomized algorithm generating
  %that sequence, is
  as
\[
\paren{1-\frac{1}{e}} \cdot \max_{\assignment \in \Feasible} \set { \sum_{\roundindex =
  1}^{\NumRounds} f_{\roundindex}(\assignment) }
\ - \
\expt{\sum_{\roundindex = 1}^{\NumRounds} f_{\roundindex}(\assignment_{\roundindex}) } \mbox { .}
\]
\ignore{
Incorporating features, we similarly define the \emph{feature-weighted}
\emph{$(1-1/e)$-regret} as
\[
\max_{\text{feature }q \in \bracket{\NumFeatures}} \left\{ \paren{1-\frac{1}{e}} \cdot \max_{\assignment \in \Feasible} \sum_{\roundindex =
  1}^{\NumRounds} \features^{\roundindex}_{q} \cdot f_{\roundindex}(\assignment)
\quad - \quad
\expt{\sum_{\roundindex = 1}^{\NumRounds} \features^{\roundindex}_{q} \cdot f_{\roundindex}(\assignment_{\roundindex})}    \right\}
\]
} % end ignore
%\end{defn}
Our goal is then to develop efficient algorithms whose
$(1-1/e)$-regret grows sublinearly in $\NumRounds$.


\paragraph{Subsumed Models.}
Our model generalizes several common models for sponsored search ad
selection, and web search results.
These include models with \emph{click-through-rates}, in which
it is assumed that each (ad, position) pair has some probability
$p(a, \k)$ of being clicked on, and there is some monetary
reward $b(a)$ that is obtained whenever ad $a$ is clicked on.
Often, the \ctrs are assumed to be \emph{separable},
meaning $p(a, \k)$ has the functional form $\alpha(a) \cdot
\beta(\k)$ for some functions $\alpha$ and $\beta$.
%This is the case in~\cite{abrams07,aggarwal06,edelman07a}.
%meaning that $p(a,j) = \alpha(a) \cdot \beta(j)$, where $\beta(j)$ is non-decreasing as a function of position.
See~\cite{feldman08,lahaie07} for more details on
sponsored search ad allocation.  Note that in both of these cases, the
(expected) reward of a set $S$ of (ad, position) pairs
is $\sum_{(a,\k) \in S}{g(a,\k)}$ for some nonnegative function $g$.
It is easy to verify that such a reward function is monotone submodular.
Thus, we can capture this model in our framework by setting $\Partition_\k = \mathcal{A} \times \set {\k}$, where $\mathcal{A}$ is the set of ads.
Another subsumed model, for web search, appears in~\cite{radlinski08};
it assumes that each user is interested in a particular set of
results, and any list of results that intersects this set generates a unit
of value; all other lists generate no value (the ordering of results is irrelevant).  Again, the reward function is monotone submodular.
In this setting, it is desirable to display a diverse set of results in order to maximize the likelihood that at least one of them will interest the user.
%For this particular
%model the ordering of results is irrelevant, and thus the algorithm in~\cite{streeter08} gives
%similar results to ours.  However, unlike the algorithm
%in~\cite{streeter08} our algorithm can handle various kinds of
%position dependence in the reward function.

Our model is flexible in that we can handle position-dependent effects and diversity considerations simultaneously.  For example, we can
handle the case that each user $u$ is interested in a particular set $A_u$ of ads
and looks at a set $I_u$ of positions, and the reward of an assignment $\assignment$ is
any monotone-increasing concave function $g$ of $|\assignment \cap (A_u \times I_u)|$.  If $I_u = \set {1, 2, \ldots, k}$ and $g(x) = x$, this models the case where the quality is the number of relevant result
that appear in the first $k$ positions.
If $I_u$ equals all positions and $g(x) = \min \set{x, 1}$ we recover the model of~\cite{radlinski08}.








==> macros.tex <==


\newcommand{\daniel}[1]{}
\newcommand{\matt}[1]{}
%\newcommand{\andreas}[1]{}
%\newcommand{\daniel}[1]{\textcolor{blue}{Daniel: #1}}
%\newcommand{\matt}[1]{\textcolor{red}{Matt: #1}}
\newcommand{\andreas}[1]{\textcolor{green}{Andreas: #1}}

\newcommand{\myskip}{\myvspace{-1mm}}

\newcommand{\cf}{\emph{c.f.}}

\newcommand{\captionsmall}[1]{\caption{\small #1}}
\newcommand{\commentout}[1]{}

\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cC}{{\mathcal{C}}}

\newcommand{\scen}{{\mathcal{I}}}

\newcommand{\balpha}{{\mathbf{\alpha}}}
\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bh}{{\mathbf{h}}}
\newcommand{\bs}{{\mathbf{s}}}
\newcommand{\bt}{{\mathbf{t}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bv}{{\mathbf{v}}}
\newcommand{\bw}{{\mathbf{w}}}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\bz}{{\mathbf{z}}}


% Dan's Macros
% ==============================================

\newenvironment{Enum}{
\vspace{-0.5em}
\begin{enumerate}
   \setlength{\itemsep}{0.25em}%{3pt}
  \setlength{\parskip}{0em}
  \setlength{\parsep}{0em}}
{\end{enumerate}\vspace{-0.5em}}

\newcounter{myLISTctr}
\newcommand{\initOneLiners}{%
    \setlength{\itemsep}{0pt}
    \setlength{\parsep }{0pt}
    \setlength{\topsep }{0pt}
%      \usecounter{myLISTctr}
}
\newenvironment{OneLiners}[1][\ensuremath{\bullet}]
    {\begin{list}
        {#1}
        {\initOneLiners}}
    {\end{list}}

\newcommand{\ignore}[1]{}

\def \etal {\emph{et al.}\ }
\def \argmax {\mathop{\rm arg\,max}}
\def \argmin {\mathop{\rm arg\,min}}

\newcommand{\ith}{\ensuremath{i^{\mathrm{th}}}\xspace}
\newcommand{\jth}{\ensuremath{j^{\mathrm{th}}}\xspace}


% basics
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\paren} [1] {\ensuremath{ \left( {#1} \right) }}
\newcommand{\bigparen} [1] {\ensuremath{ \Big( {#1} \Big) }}
%\newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}}
\renewcommand{\Pr}[1]{\ensuremath{\mathbb{P}\left[#1\right] }}
\newcommand{\E}[1]{\ensuremath{\mathbb{E}\left[#1\right] }}
%\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\size}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil#1\right\rceil}}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor#1\right\rfloor}}
%\newcommand{\norm}[2]{\ensuremath{\Vert {#1} \Vert_{#2}}}
\newcommand{\tuple}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\func}[3]{\ensuremath{#1 : #2 \rightarrow #3}}
\newcommand{\problem} [1] {{\sc #1}}

% sets
\newcommand{\integers}{\ensuremath{\mathbb{Z}}}
\newcommand{\nats}{\ensuremath{\mathbb{N}}}
\newcommand{\reals}{\ensuremath{\mathbb{R}}}

% asymptotics
\newcommand{\littleO}[1]{\ensuremath{o\paren{#1}}}
\newcommand{\bigO}[1]{\ensuremath{O\paren{#1}}}
\newcommand{\bigTheta}[1]{\ensuremath{\Theta\paren{#1}}}
\newcommand{\bigOmega}[1]{\ensuremath{\Omega\paren{#1}}}

% complexity classes
\newcommand{\class} [1] {\textrm{#1}} % bf or sc or rm?
\renewcommand{\P} {\class{P}}
\newcommand{\NP} {\class{NP}}

% specific to this paper

% Conventions:
% ===================================================
% use t to index rounds.
% use i to index partitions, j to index colors
% use capital letters for sets, lower case for elements
% ===================================================
\newcommand{\roundindex}{\ensuremath{t}}
\newcommand{\partitionindex}{\ensuremath{k}}


\newcommand{\features}{\ensuremath{v}}
\newcommand{\NumFeatures}{\ensuremath{m}}
\newcommand{\NumRounds}{\ensuremath{T}}

\newcommand{\colorindex}{\ensuremath{c}}
\newcommand{\Color}{\ensuremath{c}}
\newcommand{\Colors}{\ensuremath{\bracket{\NumColors}}}
\newcommand{\Colorvec}{\ensuremath{ \vec{c} }}

\def \k {\partitionindex}
\def \c {\colorindex}
\def \cvec {\Colorvec}
\def \j {\c}
\def \t {\roundindex}
\def \C {\NumColors}
\def \J {\C}
\def \K {\NumPartitions}
\def \P {\Partition}
\def \T {\NumRounds}
% Conventions:
% use \t to index rounds.
% use \k to index partitions, \c to index colors
% use capital letters for sets, lower case for elements
% ========= End Matt's Macros ================================

% ===================================================


\newcommand{\assignment}{S}  % Matt: I changed from \cS to just S, which I
% think is better.  If you change this back, please update the algorithms
% section to use this macro so that notation will be consistent.

%\newcommand {\positions}{\ensuremath{\cW}} %{\ensuremath{X}}
\newcommand {\groundset}{\ensuremath{\cV}} %{\ensuremath{X}}
\newcommand {\groundsettimespartitions}{\ensuremath{\groundset\times\bracket{\NumPartitions}}} %{\ensuremath{X}}
\newcommand {\matroidgroundset}{\ensuremath{\mathcal{X}}}
 %{\ensuremath{\mathcal{X_{\matroid}}}}
\newcommand {\listgroundset} {\ensuremath{U}}
\newcommand{\OPT}{\textsf{OPT}}
\newcommand{\NULL}{\textsf{null}}

\newcommand{\obj}{\ensuremath{f}} % objective function

\newcommand{\matroid}{\ensuremath{\mathcal{M}}}
%\newcommand{\indset}{\ensuremath{\mathcal{I}}}

\newcommand{\setoflist}[1]{\ensuremath{\operatorname{set}({#1})}}
\newcommand{\listofset}[1]{\ensuremath{\operatorname{list}({#1})}}
\newcommand {\ctr} {click-through-rate\xspace}
\newcommand {\ctrs} {click-through-rates\xspace}

% ========== end Dan's macros ======================================


% ========= Matt's Macros ================================
\newcommand{\omitproof}[1]{}

\newcommand{\bracket}[1]{\left[#1\right]}
\newcommand{\Esub}[2]{\mathbb{E}_{#1}\bracket{#2}}
\newcommand{\sample}{\textsf{sample}}

\newcommand{\Alg}{\ensuremath{\mathcal{E}}}
\newcommand{\AllRows}{\ensuremath{\mathcal{R}_{\bracket{\J}}}}

\newcommand {\Feasible} {\mathcal{P}}
\newcommand{\LocallyGreedy}{{\bf LocallyGreedy}\xspace}
\newcommand{\NonNegativeReals}{\ensuremath{\mathbb{R}_{\ge 0}}}

\newcommand{\NumColors}{\ensuremath{C}}
\newcommand{\NumPartitions}{\ensuremath{K}}
%\newcommand{\OfflineGreedyFullName}{\sc TabularGreedy}
\newcommand{\OfflineGreedy}{{\sc TabularGreedy}\xspace}
\newcommand{\OnlineGreedy}{{\sc TGbandit}\xspace}
\newcommand{\Partition}{\ensuremath{P}}
\newcommand{\Regret}{\ensuremath{r}}
\newcommand{\Row}{\ensuremath{R}}
\newcommand{\Rows}{\ensuremath{\mathcal{R}}}
\newcommand{\SubGreedy}{{\bf SubGreedy}\ }



% ----------------------------------------------------------------
\vfuzz2pt % Don't report over-full v-boxes if over-edge is small
\hfuzz2pt % Don't report over-full h-boxes if over-edge is smallq
% THEOREMS -------------------------------------------------------
\newtheorem{thm}{Theorem}%[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{prob}[thm]{Problem}
\newtheorem{example}[thm]{Example}
\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
\numberwithin{equation}{section}
% MATH -----------------------------------------------------------
\DeclareMathOperator{\pr}{Pr} \DeclareMathOperator{\dist}{Dist}
\DeclareMathOperator{\dom}{dom}
\newcommand{\expt}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\Real}{\mathbb R}
\newcommand{\eps}{\varepsilon}
\newcommand{\To}{\longrightarrow}
\newcommand{\BX}{\mathbf{B}(X)}
%\newcommand{\NPPP}{\mathbf{NP}^{\mathbf{PP}}}
%\newcommand{\cP}{\mathbf{P}}
%\newcommand{\cNP}{\mathbf{NP}}
\DeclareMathOperator{\cP}{P} \DeclareMathOperator{\cNP}{NP}
\DeclareMathOperator{\DTIME}{DTIME}
\newcommand{\maxmarg}{{P}^{max}}

\newcommand{\rew}{\mathfrak{R}}

\newcommand{\hpts}{\hat{p}_{t,\bs}}
\newcommand{\hps}{\hat{p}_\bs}
\newcommand{\hp}{\hat{p}}


% ----------------------------------------------------------------

\newcommand{\denselist}{
    \itemsep -2pt\topsep-8pt\partopsep-8pt
}
\newcommand{\tableref}[1]{Table~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\eqnref}[1]{Eq.~(\ref{#1})}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}


%-------------------------------------------------------------
%                       subfigure
%-------------------------------------------------------------

%% enable subfigures
%\usepackage{subfigure}

%\newbox\subfigbox
%\makeatletter
%  \newenvironment{subfloat}
%    {\def\caption##1{\gdef\subcapsave{\relax##1}}%
%     \let\subcapsave\@empty
%     \setbox\subfigbox\hbox
%       \bgroup}
%      {\egroup
%     \subfigure[\subcapsave]{\box\subfigbox}}
%\makeatother




==> online.tex <==
%\subsection {Online algorithm}

We now transform the offline algorithm of \secref {sec:offline} into
an online algorithm.  The high-level idea behind this transformation
is to replace each greedy decision made by the offline algorithm with
a no-regret online algorithm.  A similar approach was used in
\cite{radlinski08} and \cite{streeter08} to obtain an online
algorithm for different (simpler) online problems.

% Note from Matt: it may not be obvious what the possibilities for $\Alg_{i,j}$
% are.

%%%%%
\SetKw {KwEach} {each}
\begin {algorithm}
\Titleofalgo { \OnlineGreedy \ \ (described in the full-information feedback model) }
\KwIn {sets $\P_1$, $\P_2$, \ldots, $\P_\K$}
\ \\
\KwForEach $\k \in \bracket{\K}$ and $\c \in \Colors$, let $\Alg_{\k,\c}$ be
a no-regret algorithm with action set $\P_\k \times \set{\c}$. \\
\For {$t$ \KwFrom $1$ \KwTo $T$} {
  \KwForEach $\k \in \bracket{\K}$ and $\c \in \bracket {\J}$, let $g^t_{\k,\c} \in \P_\k \times \set{\c}$ be the action selected by $\Alg_{\k,\c}$ \\
    \KwForEach $\k \in \bracket{\K}$, choose $\Color_\k$ uniformly at
    random from $\bracket {\J}$.  Define $\Colorvec = (\Color_1, \ldots,
    \Color_\K)$. \\
    select the set $G_t = \sample_{\Colorvec} \paren { \set { g^t_{\k,\c}: \k \in \bracket{\K}, \c \in \bracket{\J}  } }$ \\
    observe $f_t$, and let $\bar F_t(\assignment) := f_t(\sample_{\Colorvec}(\assignment))$ \\
    \For {\KwEach $\k \in \bracket{\K}$, $\c \in \bracket{\J}$} {
    define $G^{t-}_{\k,\c} \equiv \set {g^t_{\k',\c'}:
    \k' \in \bracket{\K}, \c' < \c} \cup \set {g^t_{\k',\c}: \k' < \k }$ \\
    \KwForEach $x \in \P_\k \times \set{\c}$, feed back $\bar F_t(G^{t-}_{\k,\c} + x)$ to $\Alg_{\k,\c}$ as the reward for choosing $x$
  }
}
\end {algorithm}

The following theorem summarizes the performance of \OnlineGreedy.

%%%%%
\begin {thm} \label {thm:online_greedy}
Let $\Regret_{\k,\c}$ be the regret of $\Alg_{\k,\c}$, and let $\beta(\K,
\J) = 1 - \paren { 1 - \frac 1 \J }^\J - {\K \choose 2} \J^{-1}$.
Then
\[
    \E { \sum_{t=1}^T f_t(G_t) } \ge \beta(\K, \J) \cdot \max_{\assignment \in \Feasible} \set { \sum_{t=1}^T f_t(\assignment) } - \E { \sum_{\k=1}^\K \sum_{\c=1}^\J \Regret_{\k,\c} } \mbox { .}
\]
\end {thm}
%%%%%

Observe that Theorem \ref {thm:online_greedy} is similar to Theorem \ref {thm:offline_greedy}, with the addition of the $\E{r_{\k,\c}}$ terms.  The idea of the proof is to view \OnlineGreedy as a version of
\OfflineGreedy that, instead of greedily selecting single (element,color) pairs
$g_{\k,\c} \in \P_\k \times \set {\c}$, greedily selects (element vector,
color) pairs $\vec g_{\k,\c} \in \P_\k^T \times \set {\c}$ (this greedy decision is made with additive error $r_{\k,\c}$, which is the source of the extra terms).  Once this
correspondence is established, the theorem follows along the lines of Theorem~\ref {thm:offline_greedy}.
\ifthenelse{\boolean{istechrpt}}
{For a proof, see Appendix A.}
{For a proof, see the supplementary material \cite {supplementary}.}

\begin {cor} \label {cor:WMR}
If \OnlineGreedy is run with randomized weighted majority \cite {cesabianchi97}
as the subroutine, then
\[
    \E { \sum_{t=1}^T f_t(G_t) } \ge \beta(\K, \J) \cdot \max_{\assignment \in \Feasible} \set { \sum_{t=1}^T f_t(\assignment) } - \bigO { \J \sum_{\k=1}^\K \sqrt { T \log \size { \Partition_\k } } }  \mbox { .}
\]
where $\beta(\K, \J) = 1 - \paren { 1 - \frac 1 \J }^\J - {\K \choose
2} \J^{-1}$.
\end {cor}

Optimizing for $\J$ in Corollary~\ref{cor:WMR}
%we get
%$\J = \Theta\paren{ \frac{\K^{1/4} \sqrt{f^*}}{T^{1/4} \sum_{i=1}^\K
%\sqrt { T \log \size { \Partition_i } }} }$, which
yields $(1-\frac{1}{e})$-regret
$\tilde\Theta( \K^{3/2} T^{1/4} \sqrt{\OPT} )$ ignoring logarithmic
factors, where $\OPT := \max_{\assignment \in \Feasible} \set
{ \sum_{t=1}^T f_t(\assignment) }$ is the value of the static optimum.

\paragraph {Dealing with bandit feedback.}

\label {sec:limited_feedback}

\OnlineGreedy can be modified to work in the bandit feedback model.
The idea behind this modification is that on each round we ``explore"
with some small probability,
in such a way that on each round we obtain an unbiased estimate of the
desired feedback values $\bar F_t(G^{t-}_{\k,\c} + x)$ for each $\k \in
\bracket{\K}$, $\c \in \Colors$, and $x \in \Partition_\k$.  This
technique can be used to achieve a bound similar to the one stated in Corollary \ref {cor:WMR}, but with an additive regret term of
$\bigO{\paren{T \size{\groundset} \J \K}^\frac 2 3 \paren{\log \size{\groundset}}^\frac 1 3}$.
% Here is an informal proof of this bound.  We know from our NIPS'08 paper
% that if you take a no-regret algorithm like WMR and feed back payoffs
% between 0 and M, which are unbiased estimates of the true payoffs, then
% regret goes up by a factor of M.  Say we explore with probability $\gamma$.
% If you use the unbiased estimation procedure we implemented in our Java
% code, you get M = #(ads)*#(slots) / gamma = |V| / gamma, where V = groundset.
% So our regret will be
% M * F + gamma*T = |V| * F / gamma + gamma * T
% where F is the regret bound from the full information setting.
%
% Now, because we only explore on a gamma fraction of the rounds, when
% calculating F we can substitute gamma*T for T (I am hand-waving here, but am
% confident this is true).  Thus, we can set F = J K sqrt(gamma T log |V|).
% Substituting, we get regret bounded by
%
% |V| J K sqrt(gamma T log |V|) / gamma + gamma * T
%
% To balance these two terms, we set
%
% gamma = (|V| J K sqrt(log |V| / T))^2/3
%
% yielding regret
%
% 2 * (|V| J K sqrt(log |V| / T))^2/3 * T = (T |V| J K sqrt(log |V|))^2/3

\paragraph {Stronger notions of regret.}

By substituting in different algorithms for the subroutines
$\Alg_{\k,\c}$, we can obtain additional guarantees.  For example, Blum
and Mansour \cite {blum07} consider online problems in which we are
given \emph{time-selection functions} $I_1, I_2, \ldots, I_M$.  Each
time-selection function $I: \bracket {T} \rightarrow [0,1]$ associates
a weight with each round, and defines a corresponding weighted notion
of regret in the natural way.  Blum and Mansour's algorithm
guarantees low weighted regret with respect to all $M$ time selection
functions simultaneously.  This can be used to obtain low regret with
respect to different (possibly overlapping) windows of time
simultaneously, or to obtain low regret with respect to subsets of
rounds that have particular features.  By using their algorithm as a
subroutine within \OnlineGreedy, we get similar guarantees,
both in the full information and bandit feedback models.



==> related-work.tex <==

%There is a large literature on submodular function maximization.
For a general introduction to the literature on submodular function maximization, see~\cite{vondrak07}.  For applications of submodularity to machine
learning and AI see~\cite{krause08,krause07nearoptimal}.

Our offline problem is known as \emph{maximizing a monotone submodular
function subject to a (simple) partition matroid constraint} in the
operations research and theoretical computer science communities.
The study of this problem culminated in the elegant
$(1-1/e)$ approximation algorithm of Vondr\'{a}k~\cite{vondrak08} and
a matching unconditional lower bound of
Mirrokni~\etal~\cite{mirrokni08}.  Vondr\'{a}k's algorithm, called
the \emph{continuous-greedy algorithm}, has also been extended to
handle arbitrary matroid constraints~\cite{calinescu07}.  The
continuous-greedy algorithm, however, cannot be applied to our problem directly,
because it requires the ability to sample $f(\cdot)$ on \emph{infeasible}
sets $S \notin \Feasible$.  In our context, this means it must have
the ability to ask (for example) what the revenue will be if ads $a_1$
and $a_2$ are placed in position $\#1$
\emph{simultaneously}.
We do not know how to answer such questions in a way that leads to meaningful performance guarantees.
%We cannot gather this information, nor do we know how
%to hallucinate it in a manner that would lead to low $(1-1/e)$-regret.
%Instead, we devise a new $(1-1/e)$ approximation algorithm for
%the offline problem.

In the online setting, the most closely related work is that of
Streeter and Golovin~\cite{streeter08}.  Like us, they consider
sequences of monotone submodular reward functions that arrive online,
and develop an online algorithm that uses multi-armed bandit
algorithms as subroutines.  The key difference from our work is that,
as in \cite {radlinski08}, they are concerned with selecting a \emph
{set} of $\NumPartitions$ items rather than the more general problem
of selecting an \emph{assignment} of items to positions addressed in
this paper.  Kakade~\etal~\cite{Kakade07} considered the general
problem of using $\alpha$-approximation algorithms to construct 
no $\alpha$-regret online algorithms, and essentially proved it could 
be done for the class of linear optimization problems in which the cost function
has the form $c(S, w)$ for a solution $S$ and weight vector $w$, and 
$c(S, w)$ is linear in $w$.   However, their result is orthogonal to
ours, because our objective function is submodular and not
linear~\footnote{Of course, it is possible to linearize a submodular function by
using a separate dimension for every possible function argument, 
but this results in an exponential number of dimensions, which leads
to exponentially worse convergence time and regret bounds for the
algorithms in~\cite{Kakade07} relative to \OnlineGreedy.}.







% NOTE:
% This is not quite true, because our 2008 paper actually does allow the order to matter.
% Explain more in tech report.


%  They obtained a
%no-$(1-1/e)$-regret algorithm for the problem of
%selecting sets of bounded size online to maximize a sequence of monotone submodular
%functions.
%They also note that the $(1 - 1/e)$ factor is optimal
%for polynomial-time algorithms unless $\P = \NP$.
%Our main contribution is to obtain similar results for the more general
%case of selecting assignments under the same class of objective functions, using
%our new $(1-1/e)$ approximation algorithm for
%the offline problem.
%This generalization from sets to lists is well-motivated by the
%importance of ranking in web search, sponsored search, and other applications.
%As is the case in~\cite{streeter08}, to get results for the no-regret model, we use a no-regret algorithm for
%the \emph {non-stochastic multi-armed bandit problem}~\cite{auer2002} as a subroutine.
%Query features can be handled by using the sophisticated multi-armed bandit
%algorithms of Blum and Mansour~\cite{blum07} as a subroutine.
%For a general introduction to multi-armed bandit problems, see~\cite{blum07:AGTchapter}.




